Efficient Heterogeneous Large Language Model Decoding with Model-Attention Disaggregation

Transformer-based large language models (LLMs) exhibit impressive performance in generative tasks but also introduce significant challenges in real-world serving due to inefficient use of the expensive, computation-optimized accelerators. Although disaggregated serving architectures have been proposed to split different phases of LLM inference, the efficiency of decoding phase is still low. This is caused by the varying resource demands of different operators in the transformer-based LLMs. Specifically, the attention operator is memory-intensive, exhibiting a memory access pattern that clashes with the strengths of modern accelerators, especially for long context requests. To enhance the efficiency of LLM decoding, we introduce model-attention disaggregation. This approach leverages a collection of cheap, memory-optimized devices for the attention operator while still utilizing high-end accelerators for other parts of the model. This heterogeneous setup ensures that each component is tailored to its specific workload, maximizing overall performance and cost efficiency. Our comprehensive analysis and experiments confirm the viability of splitting the attention computation over multiple devices. Also, the communication bandwidth required between heterogeneous devices proves to be manageable with prevalent networking technologies. To further validate our theory, we develop and deploy Lamina, an LLM inference system that incorporates model-attention disaggregation in a distributed heterogeneous cluster. Experimental results indicate that Lamina can provide 16.1 ~ 90.1% higher estimated throughput than existing solutions with similar costs.

==> chapters/case.tex <==
To comprehensively understand the constraints present in current homogeneous clusters, this section will analyze the LLaMA-13B model as a representative architecture to evaluate its performance characteristics. By integrating quantitative performance models with empirical evaluations, our goal is to illustrate the substantial benefits of deploying the model across heterogeneous accelerators. This approach has the potential to significantly enhance throughput per dollar while maintaining latency at comparable levels. The specific notations used in this analysis are explained in \autoref{tab:performance-analysis-parameters}.

\begin{table}[htbp]
    \centering
    \small
    \caption{Notations used in the performance analysis. The values for LLaMA-13B are also presented.}
    \label{tab:performance-analysis-parameters}
    \begin{tabular}{c|c|c} 
        \hline
        \textbf{Parameter} & \textbf{Description}  & \textbf{Typical Value} \\ \hline
        $N$ & Number of parameters in LLM. & 13 billion \\
        $d$ & Dimension of the embeddings. & 5120 \\ 
        $L$ & Layers of the LLM. & 40 \\
        $e$ & Bytes per element. & 2 \\ \hline
        $B$ & Batch size. & $ 1 \sim 512 $ \\ 
        $l$ & Context length. & $128 \sim 4096$ \\ \hline
    \end{tabular} 
\end{table}


\subsection{Serving with a Single A100}

In our earlier discussions, we highlighted that during the decoding phase, when a batch of $B$ queries is processed, the computational tasks within each transformer block can be classified into two distinct operator types, each with significantly different arithmetic intensities. For linear transformation tasks, such as the multiplication of QKV, Out, and FFN weight matrices, the computation involves $2NB$ floating-point operations and also requires loading $e(N + Bd)$ data from global memory. This results in an arithmetic intensity of $\frac{2NB}{e(N+Bd)}$, which substantially increases with larger batch sizes. \autoref{fig:a100-linear-mfu} displays the measured results of these linear transformations executed on one A100 GPU at varying batch sizes, which demonstrates a rapid increase in MFU up to a batch size of 2048. %, thereby highlighting the benefits of increasing batch size.

\begin{figure*}[t]
    \minipage{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/a100-pure-model-mfu.pdf}
        \caption{MFU of A100 when serving the linear transformation part of the LLaMA-13B.}
        \label{fig:a100-linear-mfu}
    \endminipage\hfill
    \minipage{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/attention-percentage.pdf}
        \caption{Percentage of time consumed by attention.}
        \label{fig:attn-percent}
    \endminipage\hfill
    \minipage{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/llama7b-4080-latency.pdf}
        \caption{Scalability of RTX 4080 GPUs for serving the linear transformation part of the LLaMA-13B.}
        \label{fig:4080-scalability}
    \endminipage\hfill
    \minipage{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/attn-mbu.pdf}
        \caption{Bandwidth utilization of the attention operator with different batch sizes.}
        \label{fig:attention-mbu}
    \endminipage
\end{figure*}

% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.35\textwidth]{figures/a100-pure-model-mfu.pdf}
%     \caption{Utilization of A100 when serving the linear transformation part of the LLaMA-13B.}
%     \label{fig:a100-linear-mfu}
% \end{figure}

In contrast, the arithmetic intensity for the attention operator remains a relatively small constant. 
This is due to the attention operator's execution is essentially a group of GEMV (General Matrix-Vector Multiplication) operations, with each query independently processing its own KV cache. 
Despite advancements in optimizations allowing state-of-the-art kernels to achieve high (>80\%) model bandwidth utilization (MBU) for this operator, its MFU is generally limited to less than 5\% in most scenarios. 

% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.35\textwidth]{figures/attention-percentage.pdf}
%     \caption{Percentage of time consumed by attention.}
%     \label{fig:attn-percent}
% \end{figure}

Furthermore, as the context length increases, the proportion of time spent on attention operations also rises, leading to a decrease in overall MFU during the decoding phase. \autoref{fig:attn-percent} illustrates the proportion of time consumed by attention operators across various context lengths, using a batch size of 128 and 512. It becomes evident that attention operations dominate (exceeding 80\% of the time) when the context length surpasses 1500, a common scenario in real-world applications. 
%This trend is further corroborated by our estimation equation: XXX.
Additionally, the memory capacity required for KV cache also increases linearly with the context length. Consequently, managing a large batch size becomes impractical due to memory shortage, further diminishing the overall MFU in practical applications.

\subsection{Using Memory-Optimized Accelerators for Attention}

While numerous cost-effective accelerators offer impressive memory bandwidth and capacity, solely relying on these consumer-grade GPUs for handling large models can be insufficient. The reason lies in their limited computing power and scalability, which restricts their ability to handle the computationally intensive tasks associated with inference. For instance, a single RTX 4080 GPU is capable of delivering merely 31.2\% of the TFLOPs offered by A100. Also, as shown in \autoref{fig:4080-scalability}, using tensor parallelism with four RTX 4080 GPUs to serve a 7-billion model can achieve only 1.41$\times$ speedup against using only one GPU. For even larger models, the computation latency becomes a significant challenge, struggling to meet the QoS requirement even if more devices are used.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/llama7b-4080-latency.pdf}
%     \caption{Scalability of RTX 4080 GPUs for serving the linear transformation part of the LLaMA-13B with different batch size.}
%     \label{fig:4080-scalability}
% \end{figure}

Nevertheless, the cost-effective memory in these devices presents a feasible approach to efficiently handle the attention operator. The attention computation is highly parallelizable, as each request and each head can be processed independently. As illustrated in \autoref{fig:a100-linear-mfu}, running the attention operator with a small batch size can already saturate the entire device. Hence, it is possible to divide attention computation into smaller subtasks and distribute them across multiple cheap, memory-optimized devices without sacrificing bandwidth utilization.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/attn-mbu.pdf}
%     \caption{Bandwidth utilization of the attention operator with different batch sizes.}
%     \label{fig:attention-mbu}
% \end{figure}


\subsection{Networking Overhead Challenges}

By separating the attention operator from computation-optimized devices to memory-optimized devices, we introduce cross-machine data communications within each model layer. Even though the interconnect bandwidth in existing data centers is sufficient for attention offloading, we found that networking latency might still be a problem for efficient LLM decoding. With attention offloading, we have \emph{layer-wise data transfer} between GPUs on different nodes, which may be up to thousands round-trips per second. These frequent network transfers, if not handled in a latency-optimized way, might still significantly increase the decoding time.

The communication process between GPUs on different nodes is non-trivial. As shown in \autoref{fig:distributed-gpu-networking}, it requires the cooperation of multiple system agents (including CPU, GPU, and NIC) and consists of multiple sequentially executed steps. Specifically, when sending data in the local GPU to the remote GPU, the entire workflow typically includes the following serially performed steps. First, the CPU (1) waits for all prior kernels in GPU to finish, ensuring the data to be sent is ready. Then, it (2) copies the data to be sent from GPU to DRAM. After that, the CPU (3) enqueues a send work request to the work queue of the RDMA queue pair and (4) notify RDMA NIC to process the new work request. Finally, the NIC (5) fetches the work request from the work queue and (6) performs the data transfer to the remote node by reading the data from DRAM. Similarly, when receiving data from remote GPU, the NIC (7) writes the received data to the DRAM, and the CPU (8) waits for the completion of reception by polling the completion queue of the queue pair. Then, it (9) copies the received data to GPU and (10) launches the GPU kernels for subsequent computations. Each of these sequential steps contributes to the end-to-end communication latency. 

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/lamina-network.pdf}
    \caption{Networking workflow} \label{fig:distributed-gpu-networking}
\end{figure*}



==> chapters/introduction-old.tex <==
The emergence of transformer-based large language models (LLMs) has been attracting widespread attention due to their remarkable performance in generative tasks, including chatbots \cite{chatgpt, BingAI} and coding assistants \cite{tian2023chatgpt,githubCopilot}. The intensive computation required for these models has propelled the development of dedicated accelerators (e.g., H100, TPU v5e). These accelerators, while costly, stand out due to their unprecedented computational power measured in teraflops. In particular, these specialized accelerators often integrate high-performance computational units and high-bandwidth memories (HBM) within a single package, delivering optimal performance for large-scale model processing. In conjunction with advanced distributed training frameworks, these devices can achieve optimized model FLOPS utilization (MFU) in LLM training.

However, the ever-growing deployment of LLMs has introduced another critical challenge: the high inference costs. This challenge primarily stems from the reduced MFU during inference phases, which is a result of the unique computation pattern inherent to LLM inferences. This pattern does not align well with the capabilities of modern accelerators, leading to a significant underutilization of hardware resources.

The process of LLM inference involves two phases. The first, known as the \textit{prefill} phase, processes all input tokens from the prompt in parallel. This phase resembles the forward pass in model training and displays a high computation efficiency. However, the subsequent \textit{generation} phase, where tokens are generated sequentially one after another, requires much higher memory bandwidth. Even worse, conventional methods for enhancing GPU utilization, such as increasing batch sizes, are less effective in this phase due to the limited capacity of GPU memory.

A detailed examination reveals that the generation phase mainly comprises two types of operators, each facing distinct resource bottlenecks. Linear transformations, including QKV projections and feedforward networks, are implemented with GEMM (GEneralized Matrix-Matrix multiplication) operations. Since all requests multiply with the same parameter matrices in these operators, processing multiple requests in batch can avoid repeated parameter loads from memory, making these operators primarily computation-bound. Also, the GEMMs can be efficiently handled by specialized circuits (e.g., tensor cores) in cutting-edge accelerators. However, the self-attention operator is different. This pivotal operator requires each request to access its own, distinct data (KV cache) for computation, resulting in a batched GEMV (GEneralized Matrix-Vector multiplication) pattern. Increasing batch sizes does not reduce the bandwidth requirement but places additional pressure on the already limited memory capacity. This memory-bound workload disagrees with the inherent strengths of modern accelerators, resulting in a scenario where the memory controllers are overwhelmed while the powerful computation cores remain idle. Furthermore, as the sequence length gets longer, the size of KV caches grows proportionally, which further deteriorates the overall accelerator utilization.

\paragraph{Our contributions.}
Addressing the challenges in LLM inference has led to a plethora of solutions, ranging from model quantization and pruning to enhance performance, to system-level optimizations like continuous batching \cite{yu2022orca} and paged-attention \cite{vllm} to improve hardware utilization. Hitherto, these methods have predominantly focused on homogeneous architectures, employing only high-end flagship accelerators for inference. However, our research suggests that the unique characteristics of the LLM generation phase call for a heterogeneous architecture for better efficiency and lower cost.

We surveyed a diverse spectrum of accelerators, each distinguished by specific features ideally suited for particular aspects of LLM inference. For instance, as highlighted in \autoref{tab:memory-cost-efficiency}, consumer-grade GPUs exhibit exceptional cost-effectiveness in memory-related characteristics, providing more than $3\times$ more memory capacity and bandwidth per dollar compared to their high-end counterparts. These alternative accelerators, while falling short in raw computation power and scalability, introduce economic options for efficient handling of the attention operator. Furthermore, we anticipate that the evolution of  Processing-in-Memory (PIM) devices \cite{9749869,9251855,9895629,asifuzzaman2023survey,10.1145/3400302.3415640,9474146,10213232,10155455} will demonstrate even greater cost advantages alongside their larger capacity and higher bandwidth. Compared to conventional accelerators, PIMs provide less computation power and lack symmetric access performance to the whole memory from all computational units, but these attributes are simply not required for efficient handling of the attention operator.

\begin{table}[htbp]
    \caption{Memory specifications and cost efficiency of enterprise- and consumer-grade accelerators.}
    \label{tab:memory-cost-efficiency}
    \centering
    \small
\begin{tabular}{c|c|cc|cc} 
\hline
\multirow{3}{*}{Accelerator} & \multirow{3}{*}{Price/\$} & \multicolumn{2}{c|}{Memory Spec.}                                                                            & \multicolumn{2}{c}{Cost Efficiency} \\ \cline{3-6} 
                       &                           & \begin{tabular}[c]{@{}c@{}}Cap. \\ (GB)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Bw.\\ (GB/s)\end{tabular} & \$/GB            & \$/(GB/s)        \\
\hline
A100-80G & 17500    & 80       & 1935     & 219      & 9.04 \\
H100  & 36500    & 80       & 3350     & 456      & 10.90 \\
% MI250         & 10000    & 128      & 3277  & 78      & 3.05  \\ 
\hline
RTX 3090      & 1600     & 24        & 936.2     & 67 & 1.71 \\
RX 7900 XTX   & 1000     & 24        & 960      & 42 & 1.04 \\
Arc A770      & 350      & 16  & 560      & 22      & 0.63     \\ \hline
\end{tabular}
\end{table}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/throughput-per-cost-ctx512.pdf}
        \caption{Context length = 512}
    \end{subfigure} \hfill
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/throughput-per-cost-ctx4096.pdf}
        \caption{Context length = 4096}
    \end{subfigure}
    \caption{Relative estimated throughput per cost when serving different models, using optimal hardware configurations.}
    \label{fig:throughput-per-cost}
\end{figure}

In light of these findings, we propose an innovative concept of \textbf{attention offloading}. 
This approach involves creating two pools of accelerators --- one optimized for computational power and the other for memory bandwidth efficiency. Adopting this heterogeneous architecture allows us to design a serving system that flexibly delivers the three essential components (i.e., computational power, memory capacity, and bandwidth) for high-performance LLM inference in a cost-efficient manner. 
To demonstrate the effectiveness of our approach, \autoref{fig:throughput-per-cost} presents a comparison of estimated throughput per dollar between a traditional setup using homogeneous A100 clusters and our proposed architecture, which pairs each A100 with several memory-optimized devices. As we can see, this novel approach effectively aligns the resource demands of LLM inference with the strengths of a diverse range of hardware platforms.

More importantly, our approach not only separates accelerators into two distinct resource pools but also leads to an extremely elastic architecture. The linear transformation operators processed in the computation pool are essentially stateless operators, which facilitates natural scalability to match fluctuating workloads. This adaptability is ideal for maximizing the utilization of these precious resources.

Like other disaggregated architectures, the feasibility of our proposed attention-offloading architecture hinges on its communication demands within realistic settings. Specifically, our research aims to address two critical questions. (1) What is the minimum bandwidth requirement for interconnecting these two pools of accelerators? It would be impractical if only exceptionally high interconnect bandwidths could meet these needs. (2) While the benefits in terms of throughput are apparent in our architecture, what impact does it have on inference latency? Excessive latency could restrict the range of applicable scenarios.

Fortunately, our studies indicate that these concerns are manageable in the context of LLM inference, making it a suitable scenario for applying the disaggregated architecture. Firstly, we provide detailed profiling and a theoretical model to calculate the ratio needed for balancing between computational power and memory in varying workloads. This model also assists in determining the minimum bandwidth threshold between different accelerator pools. Our findings reveal that not only conventional system buses such as PCIe 4.0 could meet our needs, networking technologies like 200Gb Infiniband or even Ethernet, already widely deployed in current AI-oriented data centers nowadays, also suffice. The feasibility of inter-node communications for attention offloading also enables more flexible designs of disaggregated LLM inference systems.

Attention offloading may introduce additional latency due to the added overhead of scheduling and networking. To mitigate this, we have employed various techniques, such as GPUDirect RDMA and device-side busy polling, which have proven effective in reducing data transfer times. Furthermore, we have implemented communication-attention overlapping, a strategy that conceals networking time by overlapping it with attention computation. Experimental results demonstrate that our attention offloading approach can achieve latency comparable to that of existing solutions, ensuring the user experience of LLM services.

With attention offloading, the inference process with a single batch results in underutilization of resources, as the memory device remains idle when the computation device is active, and vice versa. To address this inefficiency and enhance cost-effectiveness, we introduce staggered pipelining, an advanced technique that maximizes resource utilization without compromising inference latency. Through staggered pipelining, we run multiple batches concurrently and optimize the workflow to ensure that both the computation and memory devices are engaged simultaneously, minimizing resource waste and maximizing system performance.
% This approach not only demonstrates the technical viability of our architecture but also underscores its potential to democratize large language model inference, marrying efficiency with economic feasibility.

To validate our analysis, we develop and evaluate \systemname, a distributed heterogeneous LLM inference system with attention offloading. We also conduct extensive experiments to reveal the advantages of the attention offloading architecture. Experimental results on 13B and 33B models show that our system can achieve up to 1.48$\times$–12.1$\times$ higher throughput per cost than existing solutions.



% The recently developed and deployed transformer-based large language models (LLMs) draw wide public attention because of their outstanding performance in generative natural language processing tasks. LLM-based applications, such as chatbots and coding assistants, have significantly changed various aspects of our daily lives. The computational demands for pretraining these models are substantial, which has propelled the development of dedicated accelerators. These accelerators, characterized by their formidable computation capabilities in teraflops, work in tandem with distributed frameworks to optimize the training flops utilization (MFU). Despite the advancements in training, a primary challenge arise with the widespread deployment of LLMs is minimizing inference costs. This challenge stems from the lower MFU during inference, attributed to the inherent autoregressive computation pattern of these models, which does not align well with the strengths of modern dedicated accelerators.

% Specifically, LLM inference involves two distinct computational phases. Initially, there is a prompt computation phase where input tokens are processed in parallel to generate the first output token, which resembles the forward pass in model training, achieving reasonable MFU. But, subsequently, in the token generation phase, each token is generated based on the previously generated token and cached context, exemplifying the autoregressive nature of these models.  This token generation phase is inherently more serialized. This phase is predominantly memory bandwidth and capacity-bound, as each token generation requires scanning the entire model. This scanning, if not efficiently managed, can lead to prohibitively high costs.


% The recently developed and deployed transformer-based large language models (LLMs) draw wide public attention because of their outstanding performance in generative natural language processing tasks. LLM-based applications, such as chatbots and coding assistants, have significantly changed various aspects of our daily lives. However, the unprecedented computing resources required also greatly limit the accessibility of LLM services. Reducing the cost of LLM inference is one of the primary goals of LLM researchers and practitioners.

% Compared with prior sequence models like RNN and LSTM which have fixed-length vectors as their internal states, transformer-based models have much larger states, by keeping the full history of the hidden embeddings during sequence processing. The large internal states are particularly useful for capturing long-range context dependencies, an important advantage of transformers over previous models.

% The benefits of large states in LLMs come at a cost. When serving LLMs, large-capacity memories are required to store the internal states during inference. Moreover, the memory shall provide sufficiently high bandwidth, as the whole internal states are scanned during \emph{every single} token generated by the LLM. The memory capacity and bandwidth requirements, plus the huge computing power required for executing the LLM, are three elements for efficient servings of LLMs.

% Current LLM serving systems employ hardware accelerators, such as GPUs, to aid LLM inference. The stringent GPU memory capacity greatly limits the number of concurrent requests, i.e., the batch size, which in turn limits the GPU computing power utilization.

% However, we find that no single kind of computing device can simultaneously provide high computing power, high memory capacity, and high memory bandwidth. Nevertheless, devices that achieve any two of the three elements are possible. We also find that transformer-based LLMs can be sliced into parts that require different types of computing resources. Specifically, the self-attention operators that store and scan internal states, require large memory capacity and bandwidth; the linear transformation operators that perform computation-bound matrix-matrix multiplications, require large computing power.

% Based on the above observations, we propose the idea of \emph{attention offloading}, that moves the self-attention operators to a different type of devices that provide large memory capacity and bandwidth. By taking this heterogeneous architecture, the serving system can provide all three elements required for high-performance LLM inference.

% To validate our theory, we also build \systemname, a system that offloads the attention to GPUs on the remote machines.

% In this paper, we make the following contributions:
% \begin{itemize}
%     \item We propose an extended Roofline model to analyze the performance characteristics of LLM inference systems and workloads. Using this model, we identify that the mismatch between hardware capacities and workload requirements is a main cause of the low efficiency of existing systems.
%     \item We present attention offloading, that moves the memory-intensive part of LLM inference to dedicated devices. This helps increase the batch size and thus improves the computing power utilization of accelerators.
%     \item We develop \systemname, a distributed system that provides efficient and economical LLM inference by adopting the attention offloading technique. We also conduct comprehensive experiments to demonstrate the effectiveness and efficiency of \systemname.
% \end{itemize}

==> chapters/offloading-old.tex <==
To leverage the strengths of cheap memory-optimized accelerators, we propose an attention offloading architecture to effectively address the distinct characteristics of the two operators in LLM inference. This novel approach separates the processing of the attention operator from the overall model evaluation. Such an architectural division is strategically designed to optimize performance by selecting the most suitable hardware tailored to the requirements of each operator. In particular, we employ memory-optimized devices for computing the attention operator and computation-optimized devices for the rest of the model.

\subsection{Cost Efficiency}

The disparity in arithmetic intensity between different types of operators within LLMs is a crucial factor influencing the overall efficiency of the model inference, and it forms the basis for our proposed approach in a heterogeneous accelerator environment. To analyze the cost efficiency of attention offloading, we propose pairing the compute-optimized accelerators (e.g., A100) with memory-optimized accelerators that offer $\alpha \times$ superior memory cost efficiency. Specifically, the hardware cost of a single A100 GPU could instead be used for a collection of memory-optimized accelerators, collectively achieving an aggregated memory capacity and bandwidth that is $\alpha$ times that of a single A100. As per \autoref{tab:memory-cost-efficiency}, the value of $\alpha$ lies in $3.27\times$ -- $17.3\times$ in real-world scenarios. Due to the additional cost of ancillary facilities and management, the actual cost efficiency for heterogeneous offloading is slightly higher than $\alpha$. Hence, we conservatively take the minimum value of $\alpha = 3.27$ for analysis.

With the above definition, we calculate the optimal throughput per cost by enumerating the ratios of the two types of devices. The results presented in \autoref{fig:throughput-per-cost} indicate a $2.1\times$-- $2.8\times$ theoretical cost efficiency advantage of our attention offloading architecture than homogeneous architectures when the context length is 512. This margin is even wider for longer context lengths due to the increasing proportion of the attention in the overall computation.

\subsection{Surmounting the Communication Barriers}

One potential obstacle in implementing attention offloading lies in the necessity of data transmission between heterogeneous accelerators, which could encounter the communication wall problem. 

We conduct a quantitative analysis to determine the required interconnect bandwidth for such transfers. Say we run one iteration with batch size $B$. The minimum interconnect bandwidth required without slowing down the computation devices can be calculated as 
\begin{align*}
    \text{minimum bandwidth} &= \frac{\text{size of data to transmit}}{\text{computation time}} \\
    &= \frac{4edBL}{2NB/\mfu(B)} = \frac{2edL \cdot \mfu(B)}{N}
\end{align*}
where $\mfu(B)$ is the MFU at batch size $B$. The estimated minimum bandwidths required for different model inference configurations are calculated and presented in \autoref{tab:minimum_bandwidth}.
\begin{table}[htbp]
    \centering
    \small
    \caption{Minimum interconnect bandwidth required in GB/s.}
    \label{tab:minimum_bandwidth}
\begin{tabular}{c|cccc} \hline
Batch Size & 128 & 256 & 512 & 1024 \\ \hline
LLaMA-13B @A100 & 4.90 & 8.12 & 9.08 & 10.06 \\
LLaMA-33B @2$\times$A100 & 5.94 & 9.31 & 11.56 & 12.53 \\
LLaMA-65B @4$\times$A100 & 7.55 & 11.78 & 13.92 & 15.90  \\ \hline 
\end{tabular}
\end{table}

As evident from the data presented, the required interconnect bandwidth does not exceed 20GB/s, even when dealing with large models with batch sizes as high as 1024. This bandwidth demand can be easily met only by standard bus technologies, such as PCIe Gen 4, but also by networking solutions like 200G Ethernet. Indeed, contemporary data centers already fulfill this requirement, where each GPU is typically equipped with an exclusive 200Gbps NIC to provide sufficient networking bandwidth for training.

For memory devices, the identical interconnection bandwidth is also necessary to communicate with computational devices. Since we employ a collection of more economical yet less powerful memory devices to collaboratively compute attention, the communication bandwidth needed for each individual device is significantly smaller. Consequently, we can choose to either equip each device with a less powerful NIC or install a single shared 200Gbps NIC to serve multiple memory devices.

% Although the theoretical bandwidth appears adequate for attention offloading, the requirement network latency is rather stringent. With attention offloading, each model layer involves one communication round-trip, which requires microsecond-level networking overhead without significant impact on the inference latency. 

% Computation side --- XXXXX. Thus this is enough because in current setting each A100 is equipped with an exclusive 200Gbps NIC. Our real-world analysis also validates this result, which shows that the communication overhead can be fully overlapped by the computation.
% Memory-oriented side XXXXX. Thus, if customer GPU are used, each customer GPU only requires ordinal 10Gbps ethernet is enough.

% Moreover, as we can see from the equation, the required bandwidth decreases with the increasing of hidden dimension size.
% Thus, larger models such as LLaMa-33B and LLaMa-70B are actually more easier for offloading.

% One potential challenge with this separation approach is the need for inter-device data transfer, which may be subject to the communication wall problem. Specifically, the size of input data of Attn for one request is $3ae/2$, and the output size per request is $ae/2$. Let $I$ denote the communication bandwidth between these two kind of devices. To ensure the computing power of the computation device is fully utilized without being hindered by data transfer delays, the data transfer time should be covered by the model's computation time.  Therefore, we have $2aex/I \leq 2bx/P_{\text{compute}}$, and the minimum required interconnect bandwidth is $I \geq P_{\text{compute}}ae/b$. 

% \begin{table}[htbp]
%     \centering
%     \small
%     \caption{Minimum interconnect bandwidth required in GB/s.}
%     \label{tab:minimum_bandwidth}
% \begin{tabular}{c|ccc} \hline
%  & A100 & H100 & MI250 \\ \hline
% LLaMA-7B                    & 25.4 & 80.5 & 29.5  \\
% LLaMA-13B                   & 20.3 & 64.4 & 23.6  \\
% LLaMA-33B                   & 15.6 & 49.5 & 18.1  \\
% LLaMA-65B                   & 12.7 & 40.2 & 14.7  \\
% GPT-3                       & 8.5  & 26.8 & 9.8 \\ \hline 
% \end{tabular}
% \end{table}

% The results presented in \autoref{tab:minimum_bandwidth} demonstrate that the required bandwidth for inter-device communication is attainable using current bus technologies such as PCIe (up to 64 GB/s with PCIe 5.0 x16). Additionally, high-speed networking technologies like Infiniband and Ethernet (up to 400 Gbps) can also satisfy this bandwidth requirement. This highlights the feasibility of implementing our proposed architecture in a wide variety of formats with readily available technologies.


==> chapters/performance.tex <==
To manage the immense scale and intensive computational demands of LLM inference, along with achieving interactive-level latency in LLM serving, deploying high-powered accelerators has become a prevalent approach. To better understand the performance impediments in existing accelerator-based LLM inference systems and provide insights into system optimization strategies, we establish a quantitative performance model for LLM inference workloads.
% The notations used in this paper are listed in \autoref{tab:performance-model-parameters}.

% \subsection{Extending the Roofline Model}

% The Roofline model \cite{williams-roofline} offers an intuitive way to understand the complex interplay between hardware capabilities and software requirements. By combining the operational intensity (number of operations performed per bytes read) and computational performance (measured in Flop/s), one can estimate the peak theoretical performance as well as identify the performance bottleneck (computing power or memory bandwidth) of a system. 

% \begin{table}[htbp]
%     \centering
%     \small
%     \caption{Notations in the performance model.}
%     \label{tab:performance-model-parameters}
%     \begin{tabular}{c|c|c} 
%         \hline
%         \textbf{Category} & \textbf{Parameter} & \textbf{Description} \\ \hline
%         \multirow{3}{*}{Hardware} & $P$ & computing power (in Flop/s) \\
%         & $C$ & memory capacity \\
%         & $B$ & memory bandwidth \\ \hline
%        \multirow{4}{*}{Model} & $a$ & elements per key-value pair\\
%         & $b$ & elements in model parameters \\ 
%         & $e$ & bytes per element \\
%         & $s$ & average sequence length \\ \hline
%        \multirow{2}{*}{Metrics} & $l$ & iteration latency \\
%         & $t$ & iteration throughput \\ \hline
%        \multirow{1}{*}{Variable} & $x$ & batch size \\ \hline
%     \end{tabular} 
% \end{table}


In LLM inference, the computation primarily two kinds of operators: linear transformation (LT) and attention (Attn). For each iteration of batch size $x$, the total number of math operations, the total size of accessed memory, and the quotient of the two metrics (i.e., the arithmetic intensity) are calculated as follows\footnote{The layer normalization, activation functions, and the softmax in attention are neglected to simplify analysis.}:

\begin{table}[htbp]
    \centering
    \small
    \caption{Resource requirements for different operators.}
    \begin{tabular}{c|cc|c} \hline
         &  \textbf{LT} & \textbf{Attn} & \textbf{Overall}\\ \hline
    Math Operations & $2bx$  & $2asx$ & $2x(b+as)$\\ 
    Memory Access &  $eb$  &  $easx$ & $e(b+asx)$ \\ \hline
    Arithmetic Intensity & $2x/e$ & $2/e$ & $\frac{2x(b+as)}{e(b+asx)}$ \\ \hline
    \end{tabular}
\end{table}

\begin{table}[htbp]
    \centering
    \small
        \caption{Minimum arithmetic intensity required to saturate the computing power of different devices.}
    \label{tab:arithmetic-intensity-devices}
\begin{tabular}{cc|cc|c}
\hline
Category             & Model               & \begin{tabular}[c]{@{}c@{}}BF16\\ (TFlop/s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mem. Bw.\\ (GB/s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Min. A.I.\\ (Flop/B)\end{tabular} \\ \hline
% CPU & EPYC 9754 & 25.40 & 460.8 & 55.12 \\ \hline
\multirow{2}{*}{GPU} & A100 & 312 & 2039 & 153.0 \\
                     & H100 & 990 & 3350 & 295.5 \\ \hline
TPU                  & TPU v4 & 275 & 1200 & 229.2 \\ \hline
\end{tabular}

\end{table}

The Roofline model \cite{williams-roofline} gives a simple criterion to test whether a workload is computation-bound or memory-bound on a specific device, by comparing the arithmetic intensity of the workload with a device-specific threshold (listed in \autoref{tab:arithmetic-intensity-devices}). When a workload is memory-bound, which is generally the case for LLM inference, a larger arithmetic intensity indicates a better utilization of device computing power. Note that the arithmetic intensity of LT is proportional to the batch size in LLM inference. However, relying solely on increasing the batch size to improve the overall arithmetic intensity may face two difficulties:
\begin{enumerate}
    \item The memory capacity of accelerators is limited. A larger batch size means a larger KV cache is stored in the device memory. For example, in an LLM with 33 billion parameters, a request of sequence length 512 requires 818 MB of device memory for its KV cache. If the whole device memory of an A100-80G GPU is used to store the KV cache, it can only accommodate 98 concurrent requests, far from the number required to saturate the computing power of the GPU. In practice, the device memory for KV cache is much smaller due to the space reserved for model parameters, memory fragmentation, memory over-reservation, etc., although there are attempts to improve the memory utilization in LLM inference \cite{vllm,turbotransformers}.
    \item Even if the device memory capacity is not a problem, there exists an upper bound for the overall arithmetic intensity when the batch size increases. When the batch size is sufficiently large, the KV cache read in the attention operator dominates the total size of accessed memory, which limits the overall arithmetic intensity. The arithmetic intensity upper bound can be calculated by taking the limit:
    \begin{equation}
        \text{A.I. upper bound} = \lim_{x\to+\infty} \frac{2x(b+as)}{e(b+asx)} = \frac{2b}{eas} + \frac{2}{e}.
    \end{equation}
     The calculated upper bound is depicted in \autoref{fig:ai-upper-bound} for different models and sequence lengths. Generally, the longer the sequence length is, the more likely the inference is memory-bound. With an average sequence length of about 384, the upper bound is already below the threshold of contemporary accelerators. Again, the practically achievable arithmetic intensity is much lower due to imperfect overlapping between computation and memory access, scheduling overhead, etc.

    \begin{figure}[htbp]
        \centering
        \includegraphics[width=0.33\textwidth]{figures/ai-limit.pdf}
        \caption{The upper bound on the arithmetic intensity.}
        \label{fig:ai-upper-bound}
    \end{figure}

\end{enumerate}

Both difficulties arise from the \textbf{inherent differences between the two operators} in LLM inference. The LT operator, executing a linear transformation using a shared weight matrix across all requests, exhibits a computation-intensive nature, particularly when processing many concurrent requests in batch. Conversely, Attn is a parameter-less operator that operates on each request's own KV cache, resulting in a low, constant arithmetic intensity; thus, it is always memory-bound. Current accelerators fail to efficiently handle both types of workloads, as each demands a different optimization strategy.

% In LLM inference, there exists another potential performance limit -- the memory capacity. While it is possible to make the workload less memory-bound by increasing the batch size, the maximum batch size is limited by the memory capacity to store the KV cache. Hence, we shall extend the roofline model by adding the memory capacity limit.

% Formally, we define several parameters in the performance model, as in \autoref{tab:performance-model-parameters}. By considering the computing power, memory capacity, and memory bandwidth limits, we may derive the following program:
% \begin{equation} 
%     \begin{cases}
% a x + b \leq B l & \text{(memory bandwidth limit)} \\
% (I_1  a + I_2  b) x \leq P l  & \text{(computing power limit)} \\
% ax + b \leq C & \text{(memory capacity limit)} \\
%     \end{cases}
%     \label{eq:extended-roofline}
% \end{equation} 
% Also, we have the Little's law: 
% \begin{equation}
%     x = t \times l 
%     \label{eq:littles-law}
% \end{equation} 

% Given a latency requirement $l'$, we may maximize the throughput $t$ by varying $x$, subject to \autoref{eq:extended-roofline}, \ref{eq:littles-law}, and $l \leq l'$. We may furthermore plot the throughput-latency curve by varying $l'$.  

% \subsection{Case Study}

% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[b]{0.24\textwidth}
%         \includegraphics[width=\textwidth]{figures/throughput-latency-13b-a100-40g.pdf}
%         \caption{The throughput-latency plot.}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \includegraphics[width=\textwidth]{figures/resource-util-13b-a100-40g.pdf}
%         \caption{Resource utilization.}
%     \end{subfigure}
%     \caption{The maximum theoretical throughput at different latency requirements when serving LLaMA-13B with an A100-40G GPU, calculated with the extended Roofline model. The average sequence length is set to 512.}
%     \label{fig:model-case-13b-40g}
% \end{figure}

% \autoref{fig:model-case-13b-40g} plots the throughput-latency curve, as well as resource utilization at different latency requirements, derived from the extended Roofline model, when serving a 13-billion model with an A100-40G GPU. As we can see, the memory bandwidth is the performance bottleneck in all configurations. Although it is possible to increase the operational intensity by increasing the batch size, the memory capacity will become another bottleneck. Even when the memory capacity achieves 100\% utilization, the computation only achieves about 11\% of the total GPU TFlops, resulting in a huge resource waste. 

% The phenomenon is not special to this particular setting. \autoref{tab:results-other-settings} lists the results for other models and accelerators. Therefore, we believe that the \textbf{mismatch between the hardware capabilities and workload requirements} is an essential reason for the low efficiency of existing LLM inference systems. In particular, existing accelerators have too small memory capacities to accommodate a large batch size, in order to increase the operational intensity and improve the computing power utilization.

% \begin{table}[htbp]
%     \centering
%     \small
%         \caption{Results for other models and accelerators.}
%     \label{tab:results-other-settings}
%     \begin{tabular}{c|c}
%     TBA &  TBA \\
%     TBA & TBA
%     \end{tabular}

% \end{table}

% \subsection{Discussion}

% Like the Roofline model, our performance model only gives the \textit{peak theoretical performance}, which is always larger than the actual performance in practice. The performance gap between theory and practice may be attributed to several factors:
% \begin{itemize}
%     \item 
% \end{itemize}

